Bayesian modelling of visual discrimination learning in mice

The brain constantly turns large flows of sensory information into selective representations of the environment. It, therefore, needs to learn to process those sensory inputs that are most relevant for behaviour. It is not well understood how learning changes neural circuits in visual and decision-making brain areas to adjust and improve its visually guided decision-making. To address this question, head-fixed mice were trained to move through virtual reality environments and learn visual discrimination while neural activity was recorded with two-photon calcium imaging. Previously, descriptive models of neuronal activity were fitted to the data, which was used to compare the activity of excitatory and different inhibitory cell types. However, the previous models did not take the internal representations and learning dynamics into account. Here, I present a framework to infer a model of internal representations that are used to generate the behaviour during the task. We model the learning process from untrained mice to trained mice within the normative framework of the ideal Bayesian observer and provide a Markov model for generating the movement and licking. The framework provides a space of models where a range of hypotheses about the internal representations could be compared for a given data set.

==> 99-SAMPLE_CODE.tex <==
%%%%%%%%%%%%%%%%%%%%%
%%   FIGURE
%%%%%%%%%%%%%%%%%%%%%
\textbf{SAMPLES}

Sample Figure \ref{fig:sample_figure}. Random citation \citep{baron1997synaesthesia}


\begin{figure}[h]
\centering
\includegraphics[scale=0.6]{Fig-Sample.jpg}\captionsetup{justification=raggedright,singlelinecheck=false}
\caption{How do we process behaviorally relevant and irrelevant visual information in a complex environment? }
\label{fig:sample_figure}
\end{figure}


%%%%%%%%%%%%%%%%%%%%%
%%% TABLE
%%%%%%%%%%%%%%%%%%%%%

Sample Table \ref{tab:sample_tab}.

\begin{table} [h]
\begin{center}
\caption{Some table caption} \label{tab:sample_tab}
\begin{tabular}{|c|c||c|c|} \hline
     $v_0$ & absence of grating & $o_0$ & Absence of odors 1 and 2  \\
     $v_1$ & straight grating   & $o_1$ & Odor 1 \\
     $v_2$ & angled grating     & $o_2$ &  Odor 2 \\ \hline
\end{tabular} 
\end{center}
\end{table}



